Estimating Formation Mechanisms and Degree Distributions in Mixed Attachment Networks

Our work introduces an approach for estimating the contribution of attachment mechanisms to the formation of growing networks. We present a generic model in which growth is driven by the continuous attachment of new nodes according to random and preferential linkage with a fixed probability. Past approaches apply likelihood analysis to estimate the probability of occurrence of each mechanism at a particular network instance, exploiting the concavity of the likelihood function at each point in time. However, the probability of connecting to existing nodes, and consequently the likelihood function itself, varies as networks grow. We establish conditions under which applying likelihood analysis guarantees the existence of a local maximum of the time-varying likelihood function and prove that an expectation maximization algorithm provides a convergent estimate. Furthermore, the in-degree distributions of the nodes in the growing networks are analytically characterized. Simulations show that, under the proposed conditions, expectation maximization and maximum-likelihood accurately estimate the actual contribution of each mechanism, and in-degree distributions converge to stationary distributions.

==> pestimation.tex <==
\section{Parameter Estimation}
\label{section3}
Next, consider a sequence of networks $G_0,G_1,G_2,\ldots,G_t$. Let $\A_t=\bigcup_{i=0}^t A_i$ represent the in-degrees of the nodes that, up to time $t$, have received a connection from new nodes. 

\subsection{Non-Parametric Maximum Likelihood Estimation}
\label{section3.1}
The likelihood that an edge $(u,v)$ is formed due to a new node $u$ attaching to node $v\in V_{t-1}$ is \cite{Zhang2015}
\begin{eqnarray}
\pi_t(v\mid \alpha) &= \alpha\pa(v) + (1-\alpha)\ra(v) \nonumber\\
&= \alpha\frac{\din_{t-1}(v)}{e_{t-1}}+(1-\alpha)\frac{1}{n_{t-1}}\nonumber\\
&= \alpha\left(\frac{\din_{t-1}(v)}{e_{t-1}}-\frac{1}{n_{t-1}}\right)+\frac{1}{n_{t-1}}.\label{eq4}
\end{eqnarray}
Since preferential attachment depends on the degree of the target node, \Eref{eq4} can be written as a function of the in-degree of node $v$, with $k = \din_{t-1}(v)$, namely as

\begin{equation}
\pi_t(k\mid \alpha) = \alpha\left(\frac{k}{e_{t-1}}-\frac{1}{n_{t-1}}\right)+\frac{1}{n_{t-1}}.\label{eq5}
\end{equation}

At each time $t$, the set $\A_t$ is a random sample of length $mt$. Since the elements of $\A_t$ are independent and identically distributed (i.i.d.), according to \Eref{eq5}, the likelihood function is given by
\begin{eqnarray}
f_t(\alpha)&=\prod\limits_{k\in\A_t}\pi_t(k)\nonumber\\
&= \prod\limits_{k\in\A_t}\left[\alpha\left(\frac{k}{e_{t-1}}-\frac{1}{n_{t-1}}\right)+\frac{1}{n_{t-1}}\right].\label{eq6}
\end{eqnarray}

Note that $f_t(\alpha)$ is a polynomial in the indeterminate $\alpha$, and of order at most $mt$. If all $k\in \A_t$ satisfy $k n_{t-1} - e_{t-1} \neq 0$, then the order of $f_t(\alpha)$, denoted $\deg{f_t}(\alpha)$, is $mt$.

\begin{definition}
For a network instance $G_t$, the function $f_t$ is called the $G_t$-likelihood function. Define the maximum likelihood estimator as 
\[\hat{\alpha}=\argmax_{\alpha\in[0,1]}f_t(\alpha)\]
\end{definition}

Consider a complete graph with $N_0=3$ nodes as a seed network $G_0$. We construct a network sequence $H=\left\{G_t\right\}_{t=1}^{102}$ following the mechanisms presented in \Sref{section2} with parameters $m = 5$, $\hat{m} = 2$ and $\alpha=0.75$.

Based on previous likelihood analysis \cite{Zhang2015} we consider two snapshot from $H$, and let the network evolve up to $t=101$ and $t=102$. Using \Eref{eq6} we construct the likelihood function considering the next two approximations:

\begin{description}
\item[1.] $\mathcal{A}=A_{102}$.
\item[2.] $\A_t=\bigcup_{i=0}^{102} A_i$
\end{description}

As \Fref{fig:figure2} shows, in both cases is not possible to guarantee the existence of the $\argmax$ for the likelihood function owing to the functions do not yields a maximum in the interval $[0, 1]$.

\begin{figure}[!hbt]
	\centering
	\begin{subfigure}[\label{fig:figure2_1}]
    \centering \includegraphics[width=250pt]{figure2_1.eps}
  \end{subfigure}%

  \begin{subfigure}[\label{fig:figure2_2}]
    \centering \includegraphics[width=250pt]{figure2_2.eps}
  \end{subfigure}
\caption{Likelihood functions derived from \Eref{eq6} for the two approximations.}\label{fig:figure2}
\end{figure}

The goal is to derive conditions under which $\hat{\alpha}$ exists. The next lemmata define the relationship between the number of nodes, the number of edges, and the number of roots of the $G_t$-likelihood function. They provide conditions under which the $G_t$-likelihood function has a maximum, which guarantees that the estimate $\hat{\alpha}$ exists.

\begin{lemma}\label{lem1}
If $\deg{f_t}=mt$, then there exists $mt$ different elements in $\A_t$. Moreover, for $k\in \mathcal{A}_t$ such that $kn_{t-1}\neq e_{t-1}$, the roots of $f_t$ can be written as
\[\omega_k = \frac{e_{t-1}}{e_{t-1}-k n_{t-1}}.\]
\end{lemma}

Note that the root multiplicity of $\omega_i$ corresponds to the number of times that the value of an in-degree appears in $\A_t$.

\begin{definition}
Let $\Omega(p)$ denote the \textit{roots of a polynomial $p$}. Moreover, $\Omega^+(p)$ and $\Omega^-(p)$ denote \textit{the set of positive and negative roots of $p$}.
\end{definition}

\begin{definition}
The expression $\mu_i$ denotes \textit{the multiplicity of the root $\omega_i$}.
\end{definition}

Consider the following assumption.

\begin{description}
\item[A1.] The seed network has more than $m$ nodes, each with an in-degree of at least one.
\end{description}

\begin{lemma}\label{lem2}
If there exist some $k\in \A_t$ such that $0<k<\floor{\frac{e_{t-1}}{n_{t-1}}}$, then $\Omega^+(f_t)$ and $\Omega^-(f_t)$ are non-empty sets. Moreover, $\min \Omega^+(f_t) = 1+\frac{1}{m+\hat{m}-1}$ as $t\rightarrow\infty$.
\end{lemma}
\begin{proof}

Without loss of generality, suppose that $\deg{f_t}=mt$. By Lemma \ref{lem1}, each root of $f_t$ can be written as

\begin{equation}
\omega_k = \frac{e_{t-1}}{e_{t-1}-k n_{t-1}}.\label{eq7}
\end{equation}

Since $e_{t-1}>0$, the root $\omega_k$ is positive if and only if $e_{t-1}-k n_{t-1}> 0$, which is true for some $k$ because $0<k<\floor{\frac{e_{t-1}}{n_{t-1}}}$ by hypothesis. Hence $\Omega^+(f_t)\neq \emptyset$. Moreover, if $k=1$ then the denominator of \Eref{eq7}, yields the maximum positive integer.\\

Therefore, the minimum element of $\Omega^+(f_t)$ is 
\begin{eqnarray*}
\min \Omega^+(f_t) &=\frac{e_{t-1}}{e_{t-1}-n_{t-1}}\\
&= \frac{e_{t-1}-n_{t-1}+n_{t-1}}{e_{t-1}-n_{t-1}}\\
&= 1+\frac{n_{t-1}}{e_{t-1}-n_{t-1}}.
\end{eqnarray*}
Furthermore, note that $e_{t} = e_0+(m+\hat{m})t$ and $n_t = n_0+t$. Thus
\begin{eqnarray*}
\lim_{t\rightarrow\infty}\left(\min\Omega^+(f_t)\right) &= \lim_{t\rightarrow\infty}\left(1+\frac{n_{t-1}}{e_{t-1}-n_{t-1}}\right)\\
&= \lim_{t\rightarrow\infty}\left(1+\frac{n_0+t-1}{e_0+(m+\hat{m})(t-1)-(n_0+t-1)}\right)\\
&= 1+\frac{1}{m+\hat{m}-1}.
\end{eqnarray*}
\end{proof}


\begin{theorem}\label{thm1}
If $\Omega^+(f_t)$ and $\Omega^-(f_t)$ are non-empty, and the sum of the multiplicities of positive roots is an even number, then there exist $\omega_a\in\real^-$, $\omega_b\in\real^+$, and $c\in \real$ such that $c\in (\omega_a, \omega_b)$ is a local maximum of the $G_t$-likelihood function $f_t$.
\end{theorem}
\begin{proof}
Without loss of generality, suppose that $\deg{f_t}=mt$. Note that $f_t$ can be written as a product of factors:
\begin{eqnarray*}
f_t(\alpha) &= \prod\limits_{k\in \A_t}\frac{\alpha [k n_{t-1}-e_{t-1}]+e_{t-1}}{e_{t-1} n_{t-1}}\\
&= \left(\frac{1}{e_{t-1} n_{t-1}}\right)^{mt}\prod\limits_{k\in \A_t}\alpha [k n_{t-1}-e_{t-1}]+e_{t-1}.
\end{eqnarray*}
Using Lemma \ref{lem1}
\begin{equation*}
f_t(\alpha) = \left(\frac{1}{e_{t-1} n_{t-1}}\right)^{mt}\prod\limits_{k\in \A_t}\left(\alpha-\omega_k\right).
\end{equation*}
By the hypothesis the sets of real numbers $\Omega^+(f_t)$ and $\Omega^-(f_t)$ are finite and non-empty, thus $\max\Omega^-(f_t)$ and $\min\Omega^+(f_t)$ exist. Let $\omega_a$ represent the maximum element of $\Omega^-(f_t)$ and $\omega_b$ the minimum element of $\Omega^+(f_t)$.

The function $f_t$ is continuous and differentiable in $(\omega_a,\omega_b)$. Moreover, since $\omega_a$ and $\omega_b$ are roots of $f_t$, $f_t(\omega_a) = f_t(\omega_b) = 0$. By Rolle's Theorem, there exists a constant $c\in(\omega_a,\omega_b)$ such that $f^{\prime}(c)=0$, i.e., for $\alpha\in (\omega_a,\omega_b)$, the maximum argument of $f_t$ exists.

Next, to show that the point $(c, f_t(c))$ is a local maximum of $f_t$, consider the following cases.

\begin{description}
\item[Case 1.] Suppose that $\mu_i=1$ for each root $\omega_i\in\Omega(f_t)$. Since all the roots are simple, the function $f_t$ can be written as 
\[
f_t(\alpha) = \left(\frac{1}{e_{t-1} n_{t-1}}\right)^{mt}\prod\limits_{k\in \A_t}\left(\alpha-\omega_k\right).
\]

The derivative of $f_t$ with respect to $\alpha$ is

\begin{equation}
f^{\prime}(\alpha)=\left(\frac{1}{e_{t-1}n_{t-1}}\right)^{mt}\sum\limits_{k\in\A_t}\prod\limits_{i\in \A_t \atop i \neq k}\left(\alpha-\omega_i\right). \label{eq8}
\end{equation}

Each term in the summation is a polynomial in the indeterminate $\alpha$ and of degree $mt-1$. Let 

\begin{equation}
q_k(\alpha)=\prod_{i\in \A_t \atop i \neq k}\left(\alpha-\omega_i\right).\label{eq9}
\end{equation}

By the definition of $q_k$, the root $\omega_k\in\Omega(f_t)$ does not belong to $\Omega(q_k)$, that is, $\Omega(q_k)\subsetneq\Omega(f_t)$ for each $k\in\A_t$.

Based on \Eref{eq9,eq8} can be written as

\begin{equation}
f^{\prime}(\alpha)=\left(\frac{1}{e_{t-1}n_{t-1}}\right)^{mt}\sum\limits_{k\in\A_t}q_k(\alpha). \label{eq10}
\end{equation}

By Lemma \ref{lem1}, it is guaranteed for an in-degree $j\in \A_t$ such that $\omega_j=\omega_a$ exists. For this in-degree~$j$, there exists $q_j$ such that $\omega_a$ does not belongs to $\Omega(q_j)$. Therefore, 

\begin{equation}
f^{\prime}(\omega_a)=\left(\frac{1}{e_{t-1}n_{t-1}}\right)^{mt} q_j(\omega_a).\label{eq11}
\end{equation}

The first factor in \Eref{eq11} is positive, so the sign of $f^{\prime}(\omega_a)$ depends on the sign of $q_j(\omega_a)$. Note that the product in \Eref{eq9} can be split into two factors, The first factor contains all positive roots of $q_j$ and the second one all the negative roots of $q_j$. That is,

\begin{eqnarray}
q_j(\alpha)&=&\prod_{i\in \A_t \atop i \neq j}\left(\alpha-\omega_i\right)\nonumber\\
&=& \prod\limits_{i\neq j \atop \omega_i\in\Omega^+(q_j)}(\alpha-\omega_i)\prod\limits_{i\neq j\atop \omega_i\in\Omega^-(q_j)}(\alpha-\omega_i).\label{eq12}
\end{eqnarray}

Evaluating $q(\omega_a)$, we set

\begin{equation}
q_j(\omega_a)=\prod\limits_{i\neq j \atop \omega_i\in\Omega^+(q_j)}(\omega_a-\omega_i)\prod\limits_{i\neq j\atop \omega_i\in\Omega^-(q_j)}(\omega_a-\omega_i).\label{eq13}
\end{equation}

The factors in the second product in \Eref{eq13} are positive because $\omega_a$ is the maximum element in $\Omega(f_t)$ and $\omega_a < -\omega_i$ for all $\omega_i\in\Omega^-(q_j)$. Furthermore, by the hypothesis, the first factor is a product of an even number of negative terms, which implies that the first factor is also positive.

Similarly, by using Lemma \ref{lem1}, there exists an in-degree $j^{\prime}$ such that $\omega_{j^{\prime}}=\omega_b$, so the sign of $f^{\prime}(\omega_b)$ depends on the sign of $q_{j^{\prime}}(\omega_b)$. Using the same argument as above:

\begin{equation}
q_{j^{\prime}}(\omega_b)=\prod\limits_{i\neq j^{\prime} \atop \omega_i\in\Omega^+(q_{j^\prime})}(\omega_b-\omega_i)\prod\limits_{i\neq j^{\prime} \atop \omega_i\in\Omega^-(q_{j^\prime})}(\omega_b-\omega_i).\label{eq14}
\end{equation}

On the one hand, note that $\omega_b-\omega_i<0$ because $\omega_b$ is the minimum positive root of $f_t$ and the roots are unique. On the other hand, the number of terms in the first product in \Eref{eq14} is an odd number. Thus, this product is negative. By Lemma \ref{lem2}, all positive roots are greater than $1$, so the second product in \Eref{eq14} are positive. Consequently, $q_{j^{\prime}}(\omega_b)$ is negative. Therefore, $f^{\prime}(\omega_a)>0$ and $f^{\prime}(\omega_b)<0$. Hence, $(c,f(c))$ is a local maximum of $f_t$.

\item{\textbf{Case 2.}}
Suppose that $\mu_i\geq 1$ for all roots $\omega_i\in\Omega(f_t)$, i.e., some roots have multiplicity greater than 1. Let $\bar{\A}_t$ denote the set of elements of $\A_t$ without repetitions. Since $\mu_i\geq 1$ for all roots $\omega_i\in\Omega(f_t)$, the function $f_t$ can be written as
\[
f_t(\alpha) = \left(\frac{1}{e_{t-1} n_{t-1}}\right)^{mt}\prod\limits_{k\in \bar{\A}_t}\left(\alpha-\omega_k\right)^{\mu_i}.
\]

The derivative of $f_t$ with respect to $\alpha$ is

\begin{equation}
f^{\prime}(\alpha)=\left(\frac{1}{e_{t-1}n_{t-1}}\right)^{mt}\sum\limits_{k\in\bar{\A}_t}\left[\mu_k(\alpha-\omega_k)^{\mu_k-1}\prod\limits_{i\neq k}\left(\alpha -\omega_i\right)^{\mu_i}\right]. \label{eq15}
\end{equation}

The summands in \Eref{eq15} are polynomials, each with the same roots as $f_t$, but with multiplicity of at most $m$. As for case 1, the goal is to show that $f^{\prime}(\omega_a+\epsilon)>0$ and $f^{\prime}(\omega_b-\epsilon)<0$ for some $\epsilon>0$.

Since the elements are unique, the set $\bar{\A}_t$ can be indexed as $\bar{\A}_t=\{i_1,i_2,i_3,\ldots\}$. Expanding the second factor in \Eref{eq15}, we obtain

\begin{eqnarray}
\sum\limits_{k\in\bar{\A}_t}&\left[\mu_k(\alpha-\omega_k)^{\mu_k-1}\prod\limits_{i\neq k}\left(\alpha -\omega_i\right)^{\mu_i}\right] \\
=& \mu_{i_1}(\alpha+\omega_{i_1})^{\mu_{i_1}-1}[\left(\alpha -\omega_{i_2}\right)^{\mu_{i_2}} \left(\alpha -\omega_{i_3}\right)^{\mu_{i_3}} \cdots ]\nonumber\\
&&+\mu_{i_2}(\alpha+\omega_{i_2})^{\mu_{i_2}-1}[\left(\alpha -\omega_{i_1}\right)^{\mu_{i_1}} \left(\alpha -\omega_{i_3}\right)^{\mu_{i_3}} \cdots ]\nonumber\\
&&+\mu_{i_3}(\alpha+\omega_{i_3})^{\mu_{i_3}-1}[\left(\alpha -\omega_{i_1}\right)^{\mu_{i_1}} \left(\alpha -\omega_{i_2}\right)^{\mu_{i_2}} \cdots ] \nonumber\\
&&+\cdots \nonumber\\
=& \left[\prod\limits_{k\in\bar{\A}_t}(\alpha+\omega_k)^{\mu_k-1}\right]\sum\limits_{k\in\bar{\A}_t}\left[\mu_k\prod\limits_{i\neq k}(\alpha+\omega_i)\right].
\label{eq16}
\end{eqnarray}

Using \Eref{eq16,eq15} can be written as 

\begin{equation}
f^{\prime}(\alpha)=\left(\frac{1}{e_{t-1}n_{t-1}}\right)^{mt}\left[\prod\limits_{k\in\bar{\A}_t}(\alpha+\omega_k)^{\mu_k-1}\right]\sum\limits_{k\in\bar{\A}_t}\left[\mu_k\prod\limits_{i\neq k}(\alpha+\omega_i)\right].\label{eq17}
\end{equation}

Note that the third factor, $\sum\limits_{k\in\bar{\A}_t}\left[ \mu_k\prod\limits_{i\neq k}(\alpha+\omega_i)\right]$ in \Eref{eq17}, is equal to $\sum\limits_{k\in\bar{\A}_t}\mu_k q_k(\alpha)$.

On the one hand, $q_k(\omega_a) > 0$ if and only if $|\Omega(f_t)|$ is even. Since $q_k$ is continuous over its domain, there exist some $M>0$ and $\delta>0$ such that if $(\omega_a+\epsilon)\in\:(\omega_a-\epsilon,\omega_b+\epsilon)$ and $|(\omega_a+\epsilon)-\omega_a|<\delta$, then $q_k(\omega_a+\epsilon)>0$~\cite{Apostol1974}. The second term in \Eref{eq17} can be written as

\begin{equation}
\prod\limits_{\omega_j\in\Omega^-(f_t)}(\alpha+\omega_i)^{\mu_j-1}\prod\limits_{\omega_i\in\Omega^+(f_t)}(\alpha+\omega_i)^{\mu_i-1}.\label{eq18}
\end{equation}

The first term in \Eref{eq18} is positive when evaluated at $\omega_a+\epsilon$. The second term has the property that the sum of all exponents is an even number; evaluated at $\omega_a+\epsilon$, is also positive, so $f^\prime(\omega_a+\epsilon)>0$.

On the other hand, if $|\Omega(f_t)|$ is odd, the function $q_k$ evaluated at $\omega_a$ is negative. Using the same argument as above, it can be shown that $q_k(\omega_a+\epsilon)<0$. There exists an odd number of even multiplicities by hypothesis. Consequently, the second factor in \Eref{eq18}, evaluated at $\omega_a+\epsilon$, is negative. In each case $f^\prime(\omega_a+\epsilon)>0$.
\end{description}

Similarly, it can be shown that $f^\prime(\omega_b-\epsilon)<0$. Therefore, $(c,f(c))$ is a local maximum of $f_t$.\\
\end{proof}

Next, consider a complete graph with $N_0=3$ nodes, $m = 5$ and $\hat{m}=3$ as a seed network $G_0$. We construct a network sequence from $t=1$ to $t=2\times 10^4$ following the mechanisms presented in \Sref{section2} with parameter $\alpha=0.6$. For each time we define the $G_t$-likelihood function according to \Eref{eq8}. We estimate $\alpha$ according to Theorem \ref{thm1}. \Fref{fig:test} shows how maximizing the likelihood function yields estimates $\tilde{\alpha}$ for the parameter $\alpha$.

\begin{figure}[!hbt]
\centering
\includegraphics[width=250pt]{figure3.eps}
\caption{Convergence of the parameters associated to preferential (depicted in blue) and random (depicted in red) attachment mechanisms. Here $\alpha = 0.6$.}
\label{fig:test}
\end{figure}


\subsection{An EM Algorithm}

The Expectation-Maximization (EM) algorithm computes iteratively a maximum likelihood estimator for data with unobserved variables \cite{Dempster1977}. The basic idea is to associate with a given incomplete-data problem a complete-data problem for which the maximum likelihood estimation is tractable.

Determining the contribution of the two mechanisms to the evolution of the network is equivalent to computing the likelihood estimator for a sample that comes from a mixed distribution in which the mixture weight is unknown.

For a fixed time $t$, \Eref{eq5}, which represents the likelihood of forming an edge $(u,v)$ from the new node $u$ to node $v\in V_{t-1}$ through an attachment mechanism, can be written as
\begin{eqnarray}
\pi_t(k) &= \alpha\left(\frac{k}{e_{t-1}}-\frac{1}{n_{t-1}}\right)+\frac{1}{n_{t-1}}\nonumber\\
&= \alpha\frac{k}{e_{t-1}}+(1-\alpha)\frac{1}{n_{t-1}}.
\label{eq19}
\end{eqnarray}
Let $K_t$ be a random variable that characterizes the in-degree of the selected nodes due to an attachment mechanism up to time~$t$. Moreover, let $\mathbb{P}(x\msp\theta)$ denote the probability mass function (pmf) as a function of the parameter vector $\theta$. Notice that the set $\bar{\mathcal{A}}_t=\{k_1,\ldots,k_\ell\}$ can be considered as a sample of length $\ell$ generated by the random variable $K_t$. Based on \Eref{eq19}, the incomplete likelihood function is
\begin{eqnarray}
\log \mathbb{P}(\alpha\msp\bar{\mathcal{A}}_t)&=\sum\limits_{i=1}^{\ell}\log\pi_t(k_i)\nonumber\\
&= \sum\limits_{i=1}^{\ell}\log\left(\alpha\frac{k_i}{e_{t-1}}+(1-\alpha)\frac{1}{n_{t-1}}\right).
 \label{eq20}
\end{eqnarray}
The attachment mechanism can be seen as operating on two groups of nodes. One group represents the set of all nodes that attach tot he network based on preferential attachment and the other group represents the set of nodes that attach to the network based on random attachment. Let $Y=\left(y_{ij}\right)\in\mathbb{R}^{n\times 2}$ be an $n$ by 2 matrix where $y_{ij}=1$ if the $i$-th observation is in group $j$ ($j\in\{1,2\}$) and $0$ otherwise. The expression $y_i$ denotes the $i$-row of $Y$. The variable $y$ is an indicator variable that defines the component from which an observation arises. It is known as a latent (hidden) variable \cite{Mclachlan2007}.

Notice that $\mathbb{P}(y_{i1}=1\msp\alpha)=\alpha$ and $\mathbb{P}(y_{i2}=1\msp\alpha)=1-\alpha$. For a given $i$, the value of $y_{ij}$ is $0$ except for one component, since each observation belong to only one group. Thus the conditional probabilities of the data and the unobservable data are:
\begin{eqnarray*}
\mathbb{P}(k_i\msp y_i,\alpha)&=\left(\frac{k_i}{e_{t-1}}\right)^{y_{i1}}\left(\frac{1}{n_{t-1}}\right)^{y_{i2}}\\
\mathbb{P}(y_i\msp \alpha) &= \alpha^{y_{i1}}(1-\alpha)^{y_{i2}}.
\end{eqnarray*}

By defining $Z=(\bar{\mathcal{A}}_t,Y)$ as the complete-data, the complete log-likelihood function is given by
\begin{eqnarray}
\log \mathbb{P}(Z\msp \alpha)&=\sum\limits_{i=1}^{\ell}\log\left(\mathbb{P}(k_i\msp y_i,\vec{\alpha})\mathbb{P}(y_i\msp \vec{\alpha})\right)\nonumber\\
&= \sum\limits_{i=1}^{\ell} \log \left(\left[\alpha\frac{k_i}{e_{t-1}}\right]^{y_{i1}}\left[(1-\alpha)\frac{1}{n_{t-1}}\right]^{y_{i2}}\right)\nonumber\\
&= \sum\limits_{i=1}^{\ell}y_{i1}\log \left(\alpha\frac{k_i}{e_{t-1}}\right)+\sum\limits_{i=1}^{\ell}y_{i2}\log\left((1-\alpha)\frac{1}{n_{t-1}}\right).
\label{eq21}
\end{eqnarray}

\Eref{eq21} is linear in the unobservable data $y_{ij}$. Consider a function $Q(\alpha\msp\alpha^{(d)})$ that represents the conditional expectation given the observed data using the $d$-th fit for the unknown parameter $\alpha$. In particular,
\begin{eqnarray}
Q\left(\alpha\msp\alpha^{(d)}\right) &= \mathbb{E}\left[\log \mathbb{P}(Z)\right]\nonumber\\
&= \mathbb{E}\left[\sum\limits_{i=1}^{\ell}y_{i1}\log \left(\alpha\frac{k_i}{e_{t-1}}\right)+\sum\limits_{i=1}^{\ell}y_{i2}\log\left((1-\alpha)\frac{1}{n_{t-1}}\right)\right]\nonumber\\
&= \sum\limits_{i=1}^{\ell}\mathbb{E}\left[y_{i1}\msp \bar{\mathcal{A}}_t,\alpha\right]\log \left(\alpha\frac{k_i}{e_{t-1}}\right)+\sum\limits_{i=1}^{\ell}\mathbb{E}\left[y_{i2}\msp \bar{\mathcal{A}}_t,\alpha\right]\log\left((1-\alpha)\frac{1}{n_{t-1}}\right).
\label{eq22}
\end{eqnarray}
Let $\mathbb{E}\left[y_{ij}\msp \bar{\mathcal{A}}_t,\alpha^{(d)} \right] = y^{(d)}_{ij}$. By Bayes' Theorem,
\begin{eqnarray*}
y^{(d)}_{ij} &= \mathbb{P}\left(y_{ij}=1\msp k_i,\alpha^{(d)}\right)\nonumber\\
&= \frac{\mathbb{P}\left(k_i\msp y_{ij}=1,\alpha^{(d)}\right)\mathbb{P}\left(y_{ij}=1\msp \alpha^{(d)}\right)}{\mathbb{P}\left(k_i\msp \alpha^{(d)}\right)}.\nonumber\\
\end{eqnarray*}
In particular, for $j=1$
\begin{eqnarray}
y^{(d)}_{i1}&= \frac{\mathbb{P}\left(k_i\msp y_{i1}=1,\alpha^{(d)}\right)\mathbb{P}\left(y_{i1}=1\msp\alpha^{(d)}\right)}{\mathbb{P}\left(k_i\msp\alpha^{(d)}\right)}\nonumber\\
&=  \frac{\frac{k_i}{e_{t-1}}\alpha^{(d)}}{\frac{k_i}{e_{t-1}}\alpha^{(d)}+\frac{1}{n_{t-1}}(1-\alpha)^{(d)}}.
\label{eq23}
\end{eqnarray}
and for $j=2$
\begin{eqnarray}
y^{(d)}_{i2}&= \frac{\mathbb{P}\left(k_i\msp y_{i2}=1,\alpha^{(d)}\right)\mathbb{P}\left(y_{i2}=1\msp\alpha^{(d)}\right)}{\mathbb{P}\left(k_i\msp\alpha^{(d)}\right)}\nonumber\\
&=  \frac{\frac{1}{n_{t-1}}(1-\alpha)^{(d)}}{\frac{k_i}{e_{t-1}}\alpha^{(d)}+\frac{1}{n_{t-1}}(1-\alpha)^{(d)}}.
\label{eq24}
\end{eqnarray}
Substituting \Eref{eq23,eq24} in \Eref{eq22}, the following equation hold:
\begin{eqnarray*}
Q\left(\alpha\msp\alpha^{(d)}\right) =& \sum\limits_{i=1}^{\ell}y^{(d)}_{i1}\log \left(\alpha\frac{k_i}{e_{t-1}}\right)+\sum\limits_{i=1}^{\ell}y^{(d)}_{i2}\log\left((1-\alpha)\frac{1}{n_{t-1}}\right).
\end{eqnarray*}
Consider $x_1=\alpha$ and $x_2=1-\alpha$. In order to maximize $Q\left(\alpha\msp\alpha^{(d)}\right)$, the Lagrange multiplier $\lambda$ with the constrain $x_1+x_2=1$ is introduced with the goal of solving the following equation:
\begin{equation}
\frac{\partial}{\partial x_1}\left[\sum\limits_{i=1}^{\ell}y^{(d)}_{i1}\log \left(x_1\frac{k_i}{e_{t-1}}\right)+\sum\limits_{i=1}^{\ell}y^{(d)}_{i2}\log\left(x_2\frac{1}{n_{t-1}}\right)+\lambda(x_1+x_2-1)\right] = 0 \label{eq25}
\end{equation} 
\Eref{eq25} has the solution:
\begin{equation}
\alpha^{(d+1)} = \frac{1}{\ell}\sum\limits_{i=1}^{\ell}\frac{\frac{k_i}{e_{t-1}}\alpha^{(d)}}{\frac{k_i}{e_{t-1}}\alpha^{(d)}+\frac{1}{n_{t-1}}(1-\alpha)^{(d)}}.
\label{eq26}
\end{equation}

\Eref{eq26} is a recursive formula for estimating $\alpha$. The following algorithm provides a value for the parameter $\alpha$ based on \Eref{eq26}. 

The input of the algorithm is a matrix $(a_{ij})\in\mathbb{Z}^{\ell\times 3}$ where for a fixed $i$, the values $a_{i1}$, $a_{i2}$ and $a_{i3}$ denotes the in-degree of the target node, the number of edges and the number of nodes in the network at time $t=i$, respectively. The first five lines of the algorithm computes the probability of the new edge is forming through preferential attachment or random attachment mechanism. The rest of the algorithm updates the value of parameter $\alpha$ until a sufficiently accurate value is reached.  

\begin{algorithm}[!hbt]
\caption{EM Algorithm}\label{alg:em}
\begin{algorithmic}[1]
\renewcommand{\algorithmicrequire}{\textbf{Input:}}
\renewcommand{\algorithmicensure}{\textbf{Output:}}
\Require A $\ell\times3$ matrix $A$ of integers with $\ell > 0$, an initial value for $\alpha$ and, an error bound $\epsilon.$
\Ensure An estimate for $\alpha$.\\
$\tau = 1$\\
$S=0$
\For {$i=1$ to $\ell$}\\
\qquad$\pi_{i1}= \frac{a_{i1}}{a_{i2}}$; $\pi_{i2}= \frac{a_{i1}}{a_{i3}}$
\EndFor
\While {$\tau \geq \epsilon$}\\
\qquad$\beta = \alpha$
\For {$i=1$ to $\ell$}\\
\qquad\qquad$S = S+\frac{\pi_{i1}\alpha}{\alpha\pi_{i1}+(1-\alpha)\pi_{i2}}$
\EndFor\\
\qquad$\alpha = \frac{S}{n}$ \\
\qquad$\tau\leftarrow |\beta-\alpha|$
\EndWhile\\
\Return $\alpha$
\end{algorithmic}
\end{algorithm}

This concludes the introduction of conditions to estimate the probability of the presence of the two attachment mechanisms, and of an algorithm to estimate such a probability up to a given error bound.



